Wonderful compactifications of Bruhat-Tits buildings in the non-split case

Given an adjoint semisimple group $G$ over a local field $k$, we prove that the maximal Satake-Berkovich compactification of the Bruhat-Tits building of $G$ can be identified with the one obtained by embedding the building into the Berkovich analytification of the wonderful compactification of $G$, extending previous results of R\'emy, Thuillier and Werner. In the process, we use the characterisation of the wonderful compactification in terms of Hilbert schemes given by Brion to extend the definition of the wonderful compactification to the case of a non-necessarily split adjoint semisimple group over an arbitrary field and investigate some of its properties pertaining to rational points on the boundary. Lastly, given a finite possibly ramified Galois extension $k'/k$, we take a look at the action of the Galois group on the maximal compactification of the building of $G$ over $k'$ and check that the Galois-fixed points are precisely the limits of sequences of fixed points in the building over $k'$, though they may not lie in the Satake-Berkovich compactification of $G$ over $k$.

==> bruhat-tits.tex <==
\section{Galois-fixed points in Bruhat-Tits theory}

Let $G$ be a semisimple group over a local field $k$. For each complete non-archimedean extension $k'/k$, we denote by $\mc B(G, k')$ the Bruhat-Tits building of $G_{k'}$, as constructed in \cite{BT2}. Recall that, by \cite[5.1.2]{Rou}, we have a compatible system of embeddings $$\iota_{l, m}: \mc B(G, l) \hookrightarrow \mc B(G, m)$$ indexed by towers of non-archimedean extensions $m/l/k$. The map $\iota_{m/l}$ is  $\Gal(m/l)$-equivariant if $m/l$ is Galois.

In this section, we recall how taking Galois-fixed points affects the building, depending on the ramification of the extension.

\subsection{Unramified descent}

In the case of an unramified extension $l/k$, the fixed point set $\mc B(G, l)^{\Gal(l/k)}$ is an affine building and $\iota_{k,l}$ identifies it with the Bruhat-Tits building of $G$ \cite{PrasadUnr}. Moreover, the simplicial structure of $\mc B(G,k)$ is very easy to relate to that of $\mc B(G,l)$: The simplices of $\mc B(G,k)$ are precisely the intersections of simplices of $\mc B(G,l)$ with the fixed-point set.

\subsection{Ramification and barbs}

In the tamely ramified case, the fixed point set is still a building and identified to the Bruhat-Tits building of $G$ (see \cite{Rou} and \cite{PrasadTR}). However, the simplicial structure of $\mc B(G, k)$ does not relate to that of $\mc B(G, l)$ as neatly as in the ramified case. 

In the general case, however, the fixed point set might not be a building. It contains the building of $G$ over $k$ but may contain some extra fixed points ("barbs"). The size of these extraneous components is bounded by the wildness of the extension. Recall that, if $l/k$ is a finite Galois extension with residue characteristic $p$, then its wildness $s(l/k)$ is the $p$-adic valuation of its ramification index. Then, we have the following statement:

\begin{thm}[{\cite[Prop 5.2.7]{Rou}}]
There exists a constant $C$ depending only on the absolute rank of $G$ such that, for each non-archimedean Galois extension $l/k$, and for each $x \in \mc B(G, l)^{\Gal(l/k)}$, we have $$d(x, \mc B(G, k)) \le C s(l/k).$$
\end{thm}

\begin{ex}
Consider the case when $k = \QQ_p$, $l = \QQ_p(\sqrt p)$, and $G = SL_{2,k}$. Let $\vpi = \sqrt p$. Then, the Galois group of the extension $l/k$ is generated by the involution $\sigma: a + b\vpi \mapsto a - b \vpi$. 

Recall from \cite[II.1.1]{Arbres} that, in this case, the Bruhat-Tits building of $G$ may be described as a graph whose vertices are homothety classes of $\mc O_k$-submodules of $k^2$ of maximal rank and where two vertices $[M_1]$ and $[M_2]$ are adjacent if and only if $M_1$ and $M_2$ may be chosen in such a way that $pM_1 \subsetneq M_2 \subsetneq M_1$.
Then, the inclusion map $\iota_{k,l}: \mc B(G, k) \to \mc B(G,l)$ may be described at the level of vertices as mapping the homothety class of an $\mc O_k$-lattice $M$ of $k^2$ to the homothety class of the $\mc O_l$-lattice $M \otimes_{\mc O_k} \mc O_l$ in $l^2$. Note that, because $l/k$ is ramified, this map does not preserve adjacency. 

Consider $e_1 = \begin{pmatrix}1\\0\end{pmatrix}$ and $e_2 = \begin{pmatrix}0\\1\end{pmatrix}$. Then, the subgroup $\begin{pmatrix}1 & 0 \\ \mc O_l & 1 \end{pmatrix}$ acts transitively on the neighbours of $[\mc O_l e_1 \oplus \mc O_l e_2]$ different from $[\vpi \mc O_l e_1 \oplus \mc O_l e_2]$, hence the neighbors of $[\mc O_l e_1 \oplus \mc O_l e_2]$ are precisely $[\mc O_l \vpi e_1 \oplus \mc O_l e_2]$ and the $[\mc O_l (e_1 + t e_2) \oplus \mc O_l \vpi e_2]$ for $t \in \mc O_l^{\times}$. Because $e_1$ and $e_2$ are in $k^2$, the Galois involution fixes $[\mc O_l e_1 \oplus \mc O_l e_2]$, $[\mc O_l \vpi e_1 \oplus \mc O_l e_2]$  and fixes the lattice $[\mc O_l (e_1 + t e_2) \oplus \mc O_l \vpi e_2]$. Moreover, a quick computation proves that there are no other fixed neighbors if $p \ne 2$, but that all neighbors are fixed if $p=2$.
\end{ex}
